Thermal Image Processing via Physics-Inspired Deep Networks

We introduce DeepIR, a new thermal image processing framework that combines physically accurate sensor modeling with deep network-based image representation. Our key enabling observations are that the images captured by thermal sensors can be factored into slowly changing, scene-independent sensor non-uniformities (that can be accurately modeled using physics) and a scene-specific radiance flux (that is well-represented using a deep network-based regularizer). DeepIR requires neither training data nor periodic ground-truth calibration with a known black body target--making it well suited for practical computer vision tasks. We demonstrate the power of going DeepIR by developing new denoising and super-resolution algorithms that exploit multiple images of the scene captured with camera jitter. Simulated and real data experiments demonstrate that DeepIR can perform high-quality non-uniformity correction with as few as three images, achieving a 10dB PSNR improvement over competing approaches.

==> sup_introduction.tex <==
%
We introduced a novel thermal imaging pipeline called DeepIR that combined the physics of an uncooled microbolometer camera and regularization via deep networks.
%
We motivated our problem and demonstrated the efficacy of DeepIR with several results on simulated and real data.
%
The supplementary document provides details about the learning procedure including the specific neural network architecture, and a more detailed study of some of the real experiments.
%
We also hosted our code online\footnote{\url{https://github.com/vishwa91/DeepIR}} for further research.
